Generalization of Brady-Yong Algorithm for Fast Hough Transform to Arbitrary Image Size

Nowadays, the Hough (discrete Radon) transform (HT/DRT) has proved to be an extremely powerful and widespread tool harnessed in a number of application areas, ranging from general image processing to X-ray computed tomography. Efficient utilization of the HT to solve applied problems demands its acceleration and increased accuracy. Along with this, most fast algorithms for computing the HT, especially the pioneering Brady-Yong algorithm, operate on power-of-two size input images and are not adapted for arbitrary size images. This paper presents a new algorithm for calculating the HT for images of arbitrary size. It generalizes the Brady-Yong algorithm from which it inherits the optimal computational complexity. Moreover, the algorithm allows to compute the HT with considerably higher accuracy compared to the existing algorithm. Herewith, the paper provides a theoretical analysis of the computational complexity and accuracy of the proposed algorithm. The conclusions of the performed experiments conform with the theoretical results.

==> codes.tex <==




















%\begin{algorithm}[H]
%  \caption{Summation Constructor}\label{alg:sum-c}
%  \begin{algorithmic}[1]
%    \REQUIRE Set of patterns increased to the power of two $Pats$, original image length $n > 0$
%    \ENSURE Lists $P_i$ of pairs of summed subpatterns at each level of the algorithm
%    \FORALL{$(x_1, y_1), (x_2, y_2) \in Pats$}
%      \STATE $P_i[j] \gets (x_1, y_1), (x_1 + \lfloor \frac{x_2 - x_1}{2} \rfloor, y_1 + \lfloor \frac{y_2 - y_1}{2} \rfloor)$
%      \STATE $P_i[j] \gets (x_2 - \lfloor \frac{x_2 - x_1}{2} \rfloor, y_2 - \lfloor \frac{y_2 - y_1}{2} \rfloor), (x_2, y_2)$
%    \ENDFOR
%    \STATE $l \gets \text{length}(C)$
%    \STATE $Z \gets \text{getZarr}(C)$
%    \STATE $periods \gets []$
%    \STATE $j \gets 0$
%    \FOR{$i \gets 1$ \TO $l-1$}
%      \IF{$Z[i] = (l - i)$}
%        \STATE $periods[j] \gets i$
%        \STATE $j \gets j+1$
%      \ENDIF
%    \ENDFOR
%    \STATE $periods[j] \gets l$
%    \STATE $\text{ans} \gets \text{min}(periods)$
%    \RETURN $\text{ans}$
%  \end{algorithmic}
%\end{algorithm}

%Note that the hashes of the summed dyadic subpatterns are the coordinates of their outer pixels

\begin{algorithm}[H]
  \caption{Build\_hash\_FHT2MT}\label{alg:sum-c}
  \begin{algorithmic}[1]
%    \REQUIRE Set of hashes of patterns increased to the power of two $Pats$, Image size n>0%, original image length $n > 0$
%    \ENSURE List $H$ of pairs of summed subpatterns at each level of the algorithm
    \STATE{\textbf{Input:} List $Pats$ of hashes of patterns increased to the power of two, Image size n>0.}
    \STATE{\textbf{Output:} List $H$ of pairs of summed subpatterns at each level of the algorithm.}
    \STATE $H \gets []$
    \STATE $D_0 \gets Pats$
    
    \FOR{$i \gets 1$ \TO ${\lceil \log n\rceil}$}
        \STATE $H_i \gets \text{empty\_set}()$
        \STATE $D_{new} \gets \text{empty\_set}()$
        \FORALL{$(x_1, y_1, x_2, y_2) \in D_{i-1}$}
%        \STATE left_pat \gets (x_1, y_1, x_1 + \lfloor \frac{x_2 - x_1}{2} \rfloor, y_1 + \lfloor \frac{y_2 - y_1}{2} \rfloor)
        \STATE $left\_{pats} \gets (x_1, y_1, x_1 + \lfloor \frac{x_2 - x_1}{2} \rfloor, y_1 + \lfloor \frac{y_2 - y_1}{2} \rfloor)$
        \STATE $right\_{pats} \gets (x_2 - \lfloor \frac{x_2 - x_1}{2} \rfloor, y_2 - \lfloor \frac{y_2 - y_1}{2} \rfloor, x_2, y_2)$
        \STATE \text{add\_to\_set}($H_i$, ($left\_{pats}, right\_{pats})$))
        \STATE \text{add\_to\_set}($D_{new}$, $left\_{pats}$)
        \STATE {add\_to\_set}($D_{new}$, $right\_{pats}$):
%        \STATE $P_i[j] \gets (x_1, y_1, x_1 + \lfloor \frac{x_2 - x_1}{2} \rfloor, y_1 + \lfloor \frac{y_2 - y_1}{2} \rfloor)$
%        \STATE \text{add\_to\_set}($H_i$, $(x_2 - \lfloor \frac{x_2 - x_1}{2} \rfloor, y_2 - \lfloor \frac{y_2 - y_1}{2} \rfloor, x_2, y_2)$):
%        \STATE $P_i[j] \gets (x_2 - \lfloor \frac{x_2 - x_1}{2} \rfloor, y_2 - \lfloor \frac{y_2 - y_1}{2} \rfloor, x_2, y_2)$

%        \STATE $l \gets \text{length}(C)$
%        \STATE $Z \gets \text{getZarr}(C)$
%        \STATE $periods \gets []$
%        \STATE $j \gets 0$
%        \FOR{$i \gets 1$ \TO $l-1$}
%        \IF{$Z[i] = (l - i)$}
%            \STATE $periods[j] \gets i$
%            \STATE $j \gets j+1$
%        \ENDIF
            \ENDFOR
            \STATE $H[i] \gets H_i$
        \ENDFOR
%        \STATE $periods[j] \gets l$
%        \STATE $\text{ans} \gets \text{min}(periods)$
        \RETURN $H$
%    \ENDFOR
  \end{algorithmic}
\end{algorithm}



\begin{algorithm}[H]
  \caption{FHT2MT and FHT2MS}\label{alg: fht_update}
  \begin{algorithmic}[1]
  \REQUIRE List $H$ of sets or lists $H_i$, where each element is a hash of subpatterns, summed at the $i$-th level of the algorithm, Image $I$, Image sizes $n>0, w>0$, Set of hashes of patterns increased to the power of two $Pats$
    \ENSURE Lists $P_i$ of pairs of summed subpatterns at each level of the algorithm
%    \REQUIRE List H of sets or lists H_i, where each element is a hash of subpatterns, summed at the i-th level of the algorithm
%    \ENSURE List $H$ of pairs of summed subpatterns at each level of the algorithm
    \FOR{$i \gets 1$ \TO $n$}
        \FOR{$j \gets 1$ \TO $n$}
            \STATE $Val_{i,j,i,j} \gets I(i,j)$
        \ENDFOR
    \ENDFOR
    \FOR{$i \gets 1$ \TO ${\lceil \log n\rceil}$}
        \FORALL{$((a_{11},a_{12}, a_{13}, a_{14})), (a_{21},a_{22}, a_{23}, a_{24}))) \in H_{i}$}
        \STATE $Val_{(a_{11},a_{12},a_{23},a_{24})} \gets Val_{(a_{11},a_{12}, a_{13}, a_{14})}+Val_{(a_{21},a_{22}, a_{23}, a_{24})}$
        \ENDFOR
    \ENDFOR
    \STATE $Res \gets []$
    \STATE $i \gets 0$
    \FORALL{$P \in Pats$}
        \STATE $Res[i] \gets (P, Val_{P})$
        \STATE $i \gets i+1$
    \ENDFOR
    \RETURN $Res$
  \end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
    \caption{Algorithm $FHT2MT$}
    \label{alg:FHT2MT}
    \begin{algorithmic}[1]
        \STATE{\textbf{Input:} $w > 0,\; h > 0,\,$ image $I_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$.}
        \STATE{\textbf{Output:} Hough-image $J_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$.}
    \STATE $pl \gets Build\_hash\_FHT2MT(w, h)$
    \STATE $J \gets Calculate\_Patterns\_FHT2M(w, h, I, pl)$
    \RETURN{}
    \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
    \caption{Algorithm $FHT2MS$}
    %\label{alg:FHT2MT}
    \begin{algorithmic}[1]
        \STATE{\textbf{Input:} $w > 0,\; h > 0,\,$ image $I_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$.}
        \STATE{\textbf{Output:} Hough-image $J_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$.}
    \STATE $pl \gets Build\_hash\_FHT2MS(w, h)$
    \STATE $J \gets Calculate\_Patterns\_FHT2M(w, h, I, pl)$
    \RETURN{}
    \end{algorithmic}
\end{algorithm}


\begin{algorithm}[H]
    \caption{Algorithm $Calculate\_Patterns\_FHT2M$}
    %\label{alg:FHT2MT}
    \begin{algorithmic}[1]
        \STATE{\textbf{Input:} $w > 0,\; h > 0,\,$ image $I_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$, pl.}
        \STATE{\textbf{Output:} Hough-image $J_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$.}
    \IF{$w > 1$}
    \STATE{$w_L \leftarrow \lfloor w / 2\rfloor$}
    \STATE{$w_L \leftarrow \lfloor w / 2\rfloor$}
    \RETURN{}
    \ELSE
        \STATE{$J \leftarrow I$}
        \RETURN{}
    \ENDIF
    \end{algorithmic}
\end{algorithm}






\begin{algorithm}[H]
  \caption{Build\_hash\_FHT2MT}
  %\label{alg:sum-c}
  \begin{algorithmic}[1]
    \STATE{\textbf{Input:} $w > 0,\; h > 0,\,$ image $I_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$, pl.}
    \STATE{\textbf{Output:} Hough-image $J_{w \times h} : \mathbb{Z}^2_{w,h} \to \mathbb{A}$.}
%    \REQUIRE Set of hashes of patterns increased to the power of two $Pats$, Image size n>0%, original image length $n > 0$
%    \ENSURE List $H$ of pairs of summed subpatterns at each level of the algorithm
    \STATE $H \gets []$
    \STATE $D_0 \gets Pats$
    
    \FOR{$i \gets 1$ \TO ${\lceil \log n\rceil}$}
        \STATE $H_i \gets \text{empty\_set}()$
        \STATE $D_i \gets \text{empty\_set}()$
        \FORALL{$(x_1, y_1, x_2, y_2) \in D_{i-1}$}
        \STATE $left\_{pats} \gets (x_1, y_1, x_1 + \lfloor \frac{x_2 - x_1}{2} \rfloor, y_1 + \lfloor \frac{y_2 - y_1}{2} \rfloor)$
        \STATE $right\_{pats} \gets (x_2 - \lfloor \frac{x_2 - x_1}{2} \rfloor, y_2 - \lfloor \frac{y_2 - y_1}{2} \rfloor, x_2, y_2)$
        \STATE \text{add\_to\_set}($H_i$, ($left\_{pats}, right\_{pats})$))
        \STATE \text{add\_to\_set}($D_i$, $left\_{pats}$)
        \STATE \text{add\_to\_set}($D_i$, $right\_{pats}$):
            \ENDFOR
            \STATE $H[i] \gets H_i$
        \ENDFOR
        \RETURN $H$
  \end{algorithmic}
\end{algorithm}
